AL-Bench: A Benchmark for Automatic Logging

Logging, the practice of inserting log statements into source code, is critical for improving software reliability. Recently, language model-based techniques have been developed to automate log statement generation based on input code. While these tools show promising results in prior studies, the fairness of their results comparisons is not guaranteed due to the use of ad hoc datasets. In addition, existing evaluation approaches exclusively dependent on code similarity metrics fail to capture the impact of code diff on runtime logging behavior, as minor code modifications can induce program uncompilable and substantial discrepancies in log output semantics. To enhance the consistency and reproducibility of logging evaluation, we introduce AL-Bench, a comprehensive benchmark designed specifically for automatic logging tools. AL-Bench includes a large-scale, high-quality, diverse dataset collected from 10 widely recognized projects with varying logging requirements. Moreover, it introduces a novel dynamic evaluation methodology to provide a run-time perspective of logging quality in addition to the traditional static evaluation at source code level. Specifically, AL-Bench not only evaluates the similarity between the oracle and predicted log statements in source code, but also evaluates the difference between the log files printed by both log statements during runtime. AL-Bench reveals significant limitations in existing static evaluation, as all logging tools show average accuracy drops of 37.49%, 23.43%, and 15.80% in predicting log position, level, and message compared to their reported results. Furthermore, with dynamic evaluation, AL-Bench reveals that 20.1%-83.6% of these generated log statements are unable to compile. Moreover, the best-performing tool achieves only 21.32% cosine similarity between the log files of the oracle and generated log statements.

==> insert/dataset_diversity.tex <==
\begin{figure}
    \centering
    % \includegraphics[width=1\linewidth]
    \includegraphics[scale=0.45]
    {img/dataset_diversity.pdf}
    \caption{Size of each dataset}
    \label{fig:diversity}
\end{figure}

==> insert/dataset_size.tex <==
\begin{figure}
    \centering
    % \includegraphics[width=1\linewidth]
    \includegraphics[scale=0.35]
    {img/dataset_size.pdf}
    \caption{Size of each dataset}
    \label{fig:size}
\end{figure}

==> insert/extract_vars.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{img/extract_vars.pdf}
    \caption{Steps of Extracting Variables}
    \label{fig:extrac_vars}
\end{figure}

==> insert/log_message_BLEU.tex <==
    \begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{img/log_message_bleu.pdf}
    \caption{An example of the limitation of static evaluation, whstrictestere the BLEU of static log message is used to represent the logging quality. BLEU scores show considerable differences when evaluating the log statement in the source code and the printed runtime logs.}
    \label{fig:bleu}
    \end{figure}

==> insert/low_quality_example.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=1\linewidth]{img/low-quality-data.pdf}
    \caption{Low quality data}
    \label{fig:low_quality_data}
\end{figure}

==> insert/pic_unreachable_statements.tex <==
    \begin{figure}[t]
    \centering
    \includegraphics[scale=0.55]{img/unreachable_statements.pdf}
    \caption{An example of compilation failure: Unreachable Statements}
    \label{fig:unreachable_statements}
    \end{figure}

==> insert/static_evaluation_example.tex <==
    \begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{img/static_evaluation.pdf}
    \caption{An example of the limitation of \textit{\textbf{static evaluation}}, where only the quality of log statements is considered. It cannot assess the compilability of the code or quality of the printed runtime logs.}
    \label{fig:static_evaluation}
    \end{figure}

==> insert/static_evaluation_example_2.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{img/static_evaluation_bad_case_2.pdf}
    \caption{An example of the limitation of static evaluation. The prediction differs from the ground truth by a slight upward shift of two lines. It causes a \textit{NullPointerException} when \texttt{timer} is \texttt{null} and fails to generate logs.}
    \label{fig:static_evaluation_bad_2}
\end{figure}


==> insert/strictly_match.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=1\linewidth]{img/log_position_strict_match.pdf}
    \caption{An example of limitations of strictly match when evaluating log positions}
    \label{fig:strictly_match}
\end{figure}

==> insert/table_evluation_old_result.tex <==
\begin{table}[htbp]
\caption{Evaluation result of tools from the previous studies}
\label{table:evaluation_old_result}
% \setlength\tabcolsep{4.5pt}
\centering
\small
\scalebox{1}{
\begin{tabular}{cccc}
    \toprule
    % \multirow{1}{*}{\textbf{Method}} & \textbf{Level Accuracy}&	\textbf{Position Accuracy}&	\textbf{Static Message Accuracy}&\textbf{Dynamic Part Accuracy}\\
    \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Level Accuracy}} & \multirow{2}{*}{\textbf{Position Accuracy}} & \textbf{Log Message}\\
    & & & \textbf{Accuracy}\\
    \midrule
    \(LANCE\)   &66.24	& 65.40& 30.05 \\
    \(LEONID_s\)  &73.53	& 82.35& 35.36 \\
    \(FastLog\) & 59.63 & 58.84 & 20.90  \\
    \(UniLog\)  &	72.3&	76.9& 27.1 \\
    \bottomrule
\end{tabular}
}
\end{table}


==> insert/table_example.tex <==


\begin{table}[tbp]
\caption{Comparison on different paradigms trained on Obj.5. data}
\label{table:paradigm}
% \setlength\tabcolsep{4pt}
\centering
\scalebox{1}{
\begin{tabular}{ccccccc}
    \toprule
    \textbf{Paradigm} & \textbf{PA} &	\textbf{LA} &	\textbf{LS} & \textbf{MA} & \textbf{BLEU} & \textbf{ROUGE}\\
    \midrule
    $\text{\codellama}_\text{{ICL}}$ &   37.5	& 62.7	& 80.2 & 0.35 & 0.31 & 27.2 \\
    $\text{\codellama}_\text{{FT}}$ & 74.3 & 70.8 & 90.6 & 19.9 & 16.9 & 43.3 \\ 
    $\text{\codellama}_\text{{IFT}}$ & \textbf{77.4} & \textbf{73.4} & \textbf{92.0} & \textbf{22.3} & \textbf{20.2} & \textbf{47.3} \\ 
    \bottomrule
\end{tabular}
}
\end{table}



\begin{table}[!ht]
\resizebox{ 0.8\linewidth}{!}{ % 表格环境外部设置（头）
\begin{tabular}{|c|c|c|c|r|l|} \hline % 其中，|c|表示文本居中，文本两边有竖直表线。
aaaaa & bbbbb & ccccc & ddddd & eeeee & fffff  \\ \hline
1 & 2 & 3 & 4 & 5 & 6  \\ \hline
7 &	8 &	9 &	10 & 11 & 12\\ \hline
13 & 14 & 15 & 16 &	17 & 18\\ \hline
\end{tabular}
}% 外部环境设置（尾）

\end{table}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{img/diversity_compare.pdf}
    \caption{Diversity of dataset}
    \label{fig:diversity}
\end{figure}
\label{sec:eval:logbench}

==> insert/table_result_dynamic.tex <==
\begin{table*}[htbp]
\normalsize
\caption{Dynamic evaluation on complete logging task.}
\label{table:evaluation_results_dynamic}
% \setlength\tabcolsep{4.5pt}
\centering
\scalebox{1}{
\begin{tabular}{c|c|ccc}
    \toprule
    % \multirow{1}{*}{\textbf{Method}} & \textbf{Level Accuracy}&	\textbf{Position Accuracy}&	\textbf{Static Message Accuracy}&\textbf{Dynamic Part Accuracy}\\
    \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{
\footnotesize Compilation Success Rate}} & \multicolumn{3}{c}{\textbf{Code Output Similarity}} \\
    & & \(Precision\)  & \(Recall\)  & \(F1\)  \\
    \midrule
  \(LANCE\)     &	\textbf{14.6}\%&	0.575& 0.586& 0.580\\
  \(LEONID_m\)    &	\textbf{10.0}\%&	0.589& 0.611& 0.599\\
     \(FastLog\)  &	\textbf{19.0}\%&	0.616& 0.618& 0.616\\
  \(UniLog\)    &	\textbf{70.2}\%&	0.534& 0.541& 0.537\\
    \bottomrule
\end{tabular}
}
\end{table*}



% \begin{tabular}{ccccc}
%     \toprule
%     \multirow{1}{*}{\textbf{Method}} & \textbf{Compilation Success Rate}& \multirow{2}[*]{ \multicolumn{3}{c}{\textbf{ Code Output Similarity}}}\\
%     \midrule
%     FastLog &	22.9&	0.0& 3.5 & 6.9\\
%     LANCE   &	0.2&	0.0& 0.0 & 0.1\\
%     LEONID  &	0.4&	0.0& 0.0 & 0.1\\
%     UniLog  &	51.7&	36.3& 4.9 & 17.3 \\
%     \bottomrule
% \end{tabular}

==> sections/alter.tex <==
\subsubsection{Evaluation Data}
\label{sec:moti:dataset}
Current evaluation datasets are ad-hoc, derived from splitting the entire collected data according to loose standards. More specifically, to ensure a sufficient amount of training data, previous studies had to adopt lenient rules for data collection. Additionally, some tools, to accommodate the limitations of their backbone models, further filter out data exceeding 512 tokens in length.
These strategies compromise data quality, reducing the reliability and effectiveness of evaluation results.
For example, \textit{LANCE} adopted the strictest data collection rules among all tools, requiring a minimum of 500 commits, 10 contributors, and 10 stars, while also excluding forked repositories on GitHub~\cite{GitHub}. However, even in the \textit{LANCE} dataset, low-quality data is pervasive. As shown in Figure~\ref{fig:low_quality}, several patterns of low-quality logging practices persist. These patterns include the duplication of variables within a single log statement, creating unnecessary redundancy; the inclusion of empty strings or meaningless content, resulting in uninformative messages; excessive use of special characters or punctuation, making printed logs difficult to parse; and mismatched logging levels, where critical messages are assigned inappropriate severities, leading to misclassification~\cite{gojko2006logging, Chen2017CharacterizingAD}.
Using low-quality data as an evaluation dataset fails to produce reliable results. Such results do not align with the expectation that logging tools should generate high-quality log statements within the code.
Furthermore, to accommodate the input length limitations of these tools,  previous studies~\cite{Mastropaolo2022UsingDL, Mastropaolo2023LogSG, Xu2024UniLogAL, xie2024fastlog} have filtered out instances longer than 512 tokens. While this data-cleaning strategy reduces the complexity of evaluation data, it also introduces significant biases by excluding longer code snippets, which are common in real-world development environments. This approach simplifies the evaluation process but fails to capture the full scope of challenges that logging tools would face when dealing with complex and extended code bases. Consequently, the evaluation results may not accurately reflect the tools’ ability to handle the demands of real-world software development, where longer snippets and more intricate code structures are prevalent. Therefore, there is a pressing need for a public, large-scale, high-quality, and diverse benchmark dataset that can better represent real-world codebases and provide a standardized platform for evaluating automatic logging tools. 

\input{insert/static_evaluation_example}

\subsubsection{Evaluation Method}
\label{sec: Motivation: Evaluation Method}
The current evaluation method focuses on assessing model performance by comparing the accuracy of each log statement component (\ie position, verbosity level, message). We refer to this as \textit{\textbf{static evaluation}} in this paper. Figure \ref{fig:static_evaluation} provides an example of static evaluation to demonstrate how it works. In this example, only the verbosity level matches, so the matched level count will increase by one, and BLEU scores will be used to calculate the average score. Finally, the matched portion of each component and the average BLEU score will be combined to reflect the performance of the tools. These statistical metrics provide insights into evaluating the quality of predicted log statements; however, this approach still does not align with the goal of ensuring that the predicted log statements generate high-quality logs.

% \input{insert/log_message_BLEU}
\input{insert/pic_unreachable_statements}
\textbf{First, it cannot assess the compilability of predicted log statements.} Compilability is a fundamental requirement for generating appropriate logs. This capability ensures that log statements can be applied to the source code without introducing compilation errors, avoiding wasting developers' efforts to debug for the predicted log statements. 
However, the current evaluation methodology, which focuses solely on comparing the individual components of log statements, cannot identify predicted log statements that use undefined variables or contain incorrect code syntax which could introduce compilation errors. As shown in Figure~\ref{fig:unreachable_statements}, the predicted log statement is injected into an unreachable position. Applying static evaluation would fail to recognize that this prediction could cause compilation errors. Instead of classifying it as a completely incorrect prediction, the evaluation would count it as a level match instance and assign it a BLEU score of 55.03, contributing to the statistical value. This could introduce significant bias when evaluating the performance, appearing favorable in metrics but performing poorly in actual usage.

\textbf{Second, it cannot assess the runtime logs generated by predicted log statements. }
The goal of writing log statements is to obtain the appropriate logs during software execution so that the quality of log statement is ultimately decided by the quality of runtime logs. 
Although comparing the correctness of log statement components provides insights into assessing the quality of logs, it can introduce bias when using statistical metrics that focus solely on log statements to evaluate the performance of logging tools.
A simple example is a mismatched verbosity level between the predicted log statement and the ground truth. In a case where only the verbosity level is mismatched while the other components are exactly matched, this instance would receive a high score in static evaluation. However, in a real-world scenario, for important error logs, if the predicted level is below the threshold, the logs will not be generated, regardless of how critical the message is. Conversely, for debug logs, if the predicted level exceeds the threshold, these logs could be printed in the production environment, leading to issues such as sensitive information leakage and increased storage costs. These two situations demonstrate that even a shift in verbosity level can turn a log statement into a completely bad case.
A more complicated case is presented in Figure~\ref{fig:static_evaluation_bad_2}. Under \textit{\textbf{static evaluation}}, this prediction with only a shift in two lines in position, also could be rewarded highly in statistic metrics. 
However, it is completely incorrect: placing the log statement at line 2 risks a \textit{NullPointerException} if the \textit{timer} object is \textit{null} when \textit{timer.get()} is called. This would cause the program to crash during execution, meaning that not only would the logs fail to be generated, but the entire program could terminate unexpectedly.
In real-world scenarios, this kind of error is critical and goes unnoticed in static evaluations. While static evaluation rewards this prediction for structural correctness, it fails to account for the actual behavior of the code when executed. Therefore, this example reinforces the need for more comprehensive evaluation methods that go beyond code-level metrics and consider the real-world implications of log statements. 

In conclusion, a log statement’s quality should be determined by its ability to avoid introducing extra errors and generate meaningful, contextually appropriate logs.

    \input{insert/static_evaluation_example_2}

\begin{tcolorbox}
\textbf{Insights:} The motivating study underscores major limitations in current evaluation efforts, including the lack of a diverse, high-quality dataset and methods that do not meet real-world needs. To improve log statement evaluation, we should collect a high-quality, diverse dataset and use an execution-based method to directly evaluate the runtime logs generated by log statements.
\end{tcolorbox}

==> sections/coverletter.tex <==
\section{cover letter}

\noindent Dear Editors,

We are pleased to submit our manuscript, “AL-Bench: A Benchmark for Automatic Logging”,
to \textbf{ACM Transactions on Software Engineering and Methodology}. 

Logging plays a vital role in enhancing software reliability by enabling runtime monitoring. While recent advances in large language models demonstrate promising capabilities for automating log statement generation, existing evaluation methodologies suffer from two fundamental flaws: the reliance on ad-hoc datasets compromises the fairness of cross-study comparisons, and code similarity metrics fail to account for runtime logging behavior—particularly how code modifications induce compilation failures or semantic distortions in log outputs. These limitations undermine the validity of current performance claims and hinder systematic progress in automated logging research.

To address these challenges, we propose AL-Bench, a comprehensive benchmarking framework that establishes rigorous evaluation standards. 
AL-Bench includes a large-scale, high-quality, diverse dataset collected from 10
widely recognized projects with varying logging requirements. Moreover, it introduces a novel dynamic evaluation methodology
to provide a run-time perspective of logging quality in addition to the traditional static evaluation at source code level. 
AL-Bench reveals significant limitations in existing static evaluation, as all logging tools show average accuracy drops of 37.49\%, 23.43\%, and 15.80\% in predicting log position, level,
and message compared to their reported results. Furthermore, with dynamic evaluation, AL-Bench reveals that 20.1\%-83.6\% of these
generated log statements are unable to compile. Moreover, the best-performing tool achieves only 21.32\% cosine similarity between
the log files of the oracle and generated log statements. To summarize, this work makes the following novel contributions to quantify the journal first:

\begin{itemize}
  \item We collected a high-quality, diverse, and large-scale dataset comprising 21,804 instances from 10 popular, high-quality GitHub projects, spanning various domains with differing logging requirements.

  \item We propose a dynamic evaluation approach that reintegrates the generated log statements into projects to evaluate their printed runtime logs as a more fine-grained proxy for illustrating logging performance.

  \item We conducted a comprehensive evaluation of popular automatic logging tools and revealed the key limitations based on the analysis of the evaluation results.

  \item All the data and code for AL-Bench are publicly available, providing valuable resources for both developers and researchers to advance the field of automatic logging.
\end{itemize}

We believe this work establishes a foundational step in furthering this research direction. We appreciate your time and look forward to your insightful comments.

\noindent Yours sincerely,

\noindent Boyin Tan, Junjielong Xu, Zhouruixing Zhu, and Pinjia He
